An Architecture Framework for Complex Data Warehouses

Nowadays, many decision support applications need to exploit data that are not only numerical or symbolic, but also multimedia, multistructure, multisource, multimodal, and/or multiversion. We term such data complex data. Managing and analyzing complex data involves a lot of different issues regarding their structure, storage and processing, and metadata are a key element in all these processes. Such problems have been addressed by classical data warehousing (i.e., applied to "simple" data). However, data warehousing approaches need to be adapted for complex data. In this paper, we first propose a precise, though open, definition of complex data. Then we present a general architecture framework for warehousing complex data. This architecture heavily relies on metadata and domain-related knowledge, and rests on the XML language, which helps storing data, metadata and domain-specific knowledge altogether, and facilitates communication between the various warehousing processes.

==> abstract.tex <==
Nowadays, many decision support applications need to exploit data that are not only numerical or symbolic, but also multimedia, multistructure, multisource, multimodal, and/or multiversion. We term such data complex data. Managing and analyzing complex data involves a lot of different issues regarding their structure, storage and processing, and metadata are a key element in all these processes. Such problems have been addressed by classical data warehousing (i.e., applied to ``simple" data). However, data warehousing approaches need to be adapted for complex data.
In this paper, we first propose a precise, though open, definition of complex data. Then we present a general architecture framework for warehousing complex data. This architecture heavily relies on metadata and domain-related knowledge, and rests on the XML language, which helps storing data, metadata and domain-specific knowledge altogether, and facilitates communication between the various warehousing processes. %Finally, we enumerate the main issues in complex data warehousing.

==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  J\'{e}r\^{o}me Darmont, Omar Boussa\"{i}d, Jean-Christian Ralaivao and Kamel Aouiche\\
  \fontsize{9}{11}\selectfont
  \textit{}\\  
  \textit{ERIC, University of Lyon 2}\\
  \textit{5 avenue Pierre Mend\`{e}s-France}\\
  \textit{69676 Bron Cedex}\\
  \textit{France}\\
  \textit{Contact email: jerome.darmont@univ-lyon2.fr}\\[10pt]
  %
}

==> keywords.tex <==
Data warehousing, Complex data, XML warehousing, Metadata, Domain-specific knowledge.


==> related_work.tex <==
\section{RELATED WORK: XML WAREHOUSING}
\label{sec:RelatedWork}

A large amount of data needed in decision-making is stored using XML formats. These data are heterogeneous and unstructured, or have an incomplete, irregular, or frequently changing structure. In a decision support context, it is thus crucial to design an XML warehouse to store and manage XML data with an analysis goal in mind. In this section, we present an overview of current research on XML warehousing. 

The first two studies~\cite{BAR03,XYL01} describe an architecture for integrating XML documents and querying them. XCube~\cite{HUM03} is a set of XML-based document templates to exchange warehouse data. The last work we present~\cite{GOL01} shows how multidimensional modeling can be carried out
starting directly from an XML source.

The first example of XML data warehouse architecture we present is based on three main components~\cite{BAR03}:
\begin{enumerate}
	\item the data warehouse specification module, which allows to design the data warehouse~\cite{BAR00};
	\item the data warehouse implementation module, which is responsible for storing XML data in a relational DBMS and to manage data extraction and maintenance;
	\item the query manager module for querying the data warehouse.
\end{enumerate}
The data warehouse specification is itself stored as an XML document containing the necessary metadata. The data warehouse is seen as a set of XML materialized views that are also XML documents. Finally, a graphic tool named DAWAX helps the user in the specification of the data warehouse.

Xyleme~\cite{XYL01} is a dynamic warehouse for XML data from the web supporting query evaluation, change control (subscription and versionning mechanisms) and data integration. The system is functionally organized in four levels:
\begin{enumerate}
	\item the physical level (the Natix repository~\cite{KAN99}, which is tailored for tree-data, and an index manager);
	\item the logical level (data acquisition and query processing);
	\item the application level (change management and semantic data integration);
	\item the interface level (interface to the web and interface with Xyleme clients).		
\end{enumerate}

XCube~\cite{HUM03} is a family of XML-based document templates to exchange warehouse data. It is organized in three modules: XCubeSchema, XCubeDimension and XCubeFact. XCubeSchema is the central format for describing the multidimensional structure of the data cube: it ties together the dimensions and the measures contained in a cube. XCubeDimension is meant to formalize the dimensional structures. The cells of the cube are defined by XCubeFact. Each cell consists of two parts: dimensions representing the multidimensional coordinates and the fact values themselves. Additionally, XCube contains advanced formats (XCubeText, XCubeQuery, XCubeFunction) that we do not describe here for space reasons.

We finally present a semi-automatic approach to the conceptual design of a datamart XML source~\cite{GOL01}. XML documents have a DTD and are supposed valid. The methodology for building the datamart consists in four steps: 
\begin{enumerate}
	\item the DTD is simplified by converting the nested definition into a flat representation, grouping together the sub-elements of the DTD that have the same name, reducing unary operators to a single unary operator, and transforming all ``+'' operators into ``*'' operators;
	\item a DTD graph is created from this DTD; its vertices correspond to elements, attributes and operators in the DTD;
	\item the designer chooses one or more vertices from the DTD graph as facts; each of them becomes the root of a fact schema;
	\item for each fact, the dimensions and measures are defined from the DTD graph.
\end{enumerate}

==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{AN ARCHITECTURE FRAMEWORK\\FOR COMPLEX DATA WAREHOUSES}

